A search for instanton-induced decay of super-heavy dark matter in the Pierre Auger Observatory data

Using data collected at the Pierre Auger Observatory, we search for signatures of instanton-induced processes that would provide evidence of super-heavy particles decaying in the Galactic halo. Such particles could have been produced sufficiently during the post-inflationary epoch to match the relic abundance of dark matter inferred today. The non-observation of these signatures allows us to probe the instanton strength and to derive a bound, the best ever obtained from instanton-mediated processes, on the reduced coupling constant of gauge interactions in the dark sector: $\alpha_X \lesssim 0.09$, for $10^{9} \lesssim M_X/{\rm GeV} < 10^{19}$.

==> pos.sty.2 <==
%% pos.sty
%% Copyright 2021 SISSA Medialab
%
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   http://www.latex-project.org/lppl.txt
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
%
% This work has the LPPL maintenance status `author-maintained'.
%
% The Current Maintainer of this work is
% SISSA Medialab <info@medialab.sissa.it>
%
% This work consists of the files pos.sty, PoSlogo.pdf and PoSlogo.ps.
\NeedsTeXFormat{LaTeX2e}
\ProvidesPackage{pos} [2021/09/21 v2.2]

\RequirePackage[T1]{fontenc}
\RequirePackage[utf8]{inputenc}

\newif\ifnatbibsort\natbibsorttrue\DeclareOption{no-natbib-sort}{\natbibsortfalse}
\ProcessOptions\relax

\RequirePackage{newtxtext}
\RequirePackage{amsthm} % before newtxmath because of macro "\openbox" defined in both packages
\RequirePackage{newtxmath}
\def\mathsterling{\mbox{\textsterling}}
\def\pounds{\mbox{\textsterling}} % while waiting for new release of newtxmath from Michael Sharpe (2015/07)
\DeclareMathAlphabet{\mathfrak}{U}{euf}{m}{n}
\SetMathAlphabet{\mathfrak}{bold}{U}{euf}{b}{n}
\RequirePackage[zerostyle=e]{newtxtt}
\RequirePackage{amsmath}
\RequirePackage{graphicx}
\ifnatbibsort\RequirePackage[numbers,sort&compress]{natbib}\else\RequirePackage[numbers,compress]{natbib}\fi
\RequirePackage[font=small,labelfont=bf]{caption}
\RequirePackage{xcolor}
\definecolor{posurl}{cmyk}{.9 .9 0 0}
\RequirePackage[colorlinks=true
,urlcolor=posurl
,anchorcolor=posurl
,citecolor=posurl
,filecolor=posurl
,linkcolor=posurl
,menucolor=posurl
,linktocpage=true
,pdfa=true
]{hyperref}

\newif\ifdotoc\dotocfalse
\newif\ifemailadd\emailaddfalse
\newif\iftoccontinuous\toccontinuousfalse
\newif\ifshorttitle\shorttitlefalse
\newif\if@PoSspecialurl\@PoSspecialurlfalse

\let\oldthefootnote\thefootnote

\RequirePackage{expl3}
\RequirePackage{xparse}

\ExplSyntaxOn
%% a sequence of "authors" for the running headers
\seq_new:N \l_authors_for_head_s

%% a sequence of "superscripts"
%% (in the same order as the authors)
\seq_new:N \l_super_s

%% a sequence of "authors"
%% (in the same order as the superscripts)
\seq_new:N \l_authors_s

%% a boolean to indicate if the footnote for the speaker should be output
\bool_new:N\l_do_speaker_note_bool\bool_set_false:N\l_do_speaker_note_bool

%% a boolean to indicate authors should be manually separated by the
%% operator or automatically by "," and "and"
\bool_new:N\l_manually_separate_authors_bool\bool_set_false:N\l_manually_separate_authors_bool
\newcommand{\manuallySeparateAuthors}{\bool_set_true:N\l_manually_separate_authors_bool}

\newcommand{\speakerFlag}{\ast}


%% accumulate authors
\RenewDocumentCommand\author{som}{%
  \seq_put_right:Nn \l_authors_s {#3}
  \IfNoValueTF{#2} % test the optional argument
  { % no optional argument used

    \IfBooleanTF#1 % test if we have the "star"
    {%
      % starred form (author*) means "speaker"
      % add this author to those for the running headers
      \seq_put_right:Nn \l_authors_for_head_s {#3}

      % save the superscripts with the same order as the authors
      \seq_put_right:Nn \l_super_s {\speakerFlag}

      \bool_set_true:N\l_do_speaker_note_bool
    }
    {
      % save the superscripts with the same order as the authors
      \seq_put_right:Nn \l_super_s {{}}
    }
  }

  { % there is an optional argument
    \IfBooleanTF#1 % test if we have the "star"
    {%
      % starred form (author*) means "speaker"
      % add this author to those for the running headers
      \seq_put_right:Nn \l_authors_for_head_s {#3}

      % save the superscripts with the same order as the authors
      \seq_put_right:Nn \l_super_s {#2,\speakerFlag}

      \bool_set_true:N\l_do_speaker_note_bool
    }
    {
      % save the superscripts with the same order as the authors
      \seq_put_right:Nn \l_super_s {#2}
    }
  }
}

\tl_new:N\l_author_tl
\tl_new:N\l_superscript_tl
\int_new:N\l_num_authors_int
\str_new:N\l_au_separator_pre_str
\str_new:N\l_au_separator_post_str
\msg_new:nnn {PoS} {empty-head-authors} {No~speaker.~Please~add~a~"*"~to~the~macro~\author}
%% output
\newcommand{\printAuthors}{%

  \int_zero_new:N\l_count_authors_int
  \str_set:Nn\l_au_separator_pre_str{,}
  \str_set:Nn\l_au_separator_post_str{~}

  % the number of authors
  \int_set:Nn\l_num_authors_int{\seq_count:N\l_authors_s}

  \int_compare:nNnTF             % If
      {\l_num_authors_int}       % the length of the authors
      =                          % is equal
      {1}                        % to 1
      {                          % then output the author:
        % get the author name and superscripts
        \seq_pop_left:NN\l_authors_s\l_author_tl
        \seq_pop_left:NN\l_super_s\l_superscript_tl

        \tl_use:N\l_author_tl$^{\tl_use:N\l_superscript_tl}$

        % It would be nice to also set the running header if necessary
        % but I was not able to do it.
        % I think it is because the headers are set before \printAuthors is called,
        % so that \l_author_tl is empty when the headers are set
        %
        %% \seq_if_empty:NT\l_authors_for_head_s{
        %%   \seq_gput_right:Nn \l_authors_for_head_s {\tl_use:N\l_author_tl}
        %% }

      }
      {                          % otherwise output all
        % if the operator included the separations (",", "and")
        % simpy output the names
        \bool_if:NTF\l_manually_separate_authors_bool
        {
          \bool_do_until:nn
               {\seq_if_empty_p:N\l_authors_s}
               {
                 % get the author name and superscripts
                 \seq_pop_left:NN\l_authors_s\l_author_tl
                 \seq_pop_left:NN\l_super_s\l_superscript_tl
                 \tl_use:N\l_author_tl
                 $^{\tl_use:N\l_superscript_tl}$
               }
        }

        % otherwise separate automatically
        {
          \bool_do_until:nn
               {\seq_if_empty_p:N\l_authors_s}
               {
                 % get the author name and superscripts
                 \seq_pop_left:NN\l_authors_s\l_author_tl
                 \seq_pop_left:NN\l_super_s\l_superscript_tl

                 % step the counter
                 \int_incr:N\l_count_authors_int

                 % if we are looking at the next-to-last author,
                 % then change the separator
                 \int_compare:nNnT
                     {\l_count_authors_int}
                     =
                     {\int_eval:n{\l_num_authors_int - 1}}
                     {
                       \str_set:Nn\l_au_separator_pre_str{}
                       \str_set:Nn\l_au_separator_post_str{~and~}
                       % TODO: use {~and\nobreakspace}
                     }
                 % if we are looking at the last author,
                 % do not add anything at the end
                 \int_compare:nNnT
                     {\l_count_authors_int}
                     =
                     {\l_num_authors_int}
                     {
                       \str_set:Nn\l_au_separator_pre_str{}
                       \str_set:Nn\l_au_separator_post_str{}
                     }
                 \tl_use:N\l_author_tl
                 \str_use:N\l_au_separator_pre_str
                 $^{\tl_use:N\l_superscript_tl}$
                 \str_use:N\l_au_separator_post_str
               }
        }
      }

      % display the speaker's foonote text if needed
      \bool_if:NTF\l_do_speaker_note_bool
           {
             \begin{NoHyper}
               \renewcommand\thefootnote{$\speakerFlag$}%
               \footnotetext{Speaker}%
               \stepcounter{footnote}%
               \let\thefootnote\oldthefootnote%
             \end{NoHyper}
           }
           {
             \seq_if_empty:NT\l_authors_for_head_s{\msg_warning:nn {PoS}{empty-head-authors}}
           }
}

\newcommand{\printHeadAuthors}{%
  \seq_use:Nnnn \l_authors_for_head_s { ~and~} { ,~ } { ~and\nobreakspace }
}

\ExplSyntaxOff


\renewcommand{\baselinestretch}{1.1}\normalsize
\setlength\lineskip{1\p@}
\setlength\parindent{1.2\parindent}
\setlength\normallineskip{1\p@}
\setlength\parskip{0\p@ \@plus \p@}
\@lowpenalty   51
\@medpenalty  151
\@highpenalty 301
\widowpenalty 1000
\clubpenalty 1000
\setcounter{topnumber}{8}
\renewcommand\topfraction{.85} % default .7
\setcounter{bottomnumber}{5}
\renewcommand\bottomfraction{.6} %.2
\setcounter{totalnumber}{8}
\renewcommand\textfraction{.15}
\renewcommand\floatpagefraction{.8}
\setcounter{dbltopnumber}{3}
\renewcommand\dbltopfraction{.85}
\renewcommand\dblfloatpagefraction{.8}
\setlength{\floatsep}{12pt plus 2pt minus 4pt}
\setlength{\textfloatsep}{20pt plus 3pt minus 8pt}
\setlength{\intextsep}{12pt plus 2pt minus 4pt}
\textwidth  .72\paperwidth	% WIDTH OF TEXT, REMAINS .28% FOR MARGINS
\setlength\@tempdima{.76\paperheight}	% HEIGHT OF TEXT WITH FOOTNOTES
\divide\@tempdima\baselineskip		% EXCLUDING HEAD (AND FOOT)
\@tempcnta=\@tempdima			% rounded to integer (#lines-1)
\setlength\textheight{\@tempcnta\baselineskip}
\addtolength\textheight{\topskip}
\voffset -1in
\topmargin   .06\paperheight	% FROM TOP OF PAGE TO TOP OF HEADING (0=1inch)
\headheight  .02\paperheight	% HEIGHT OF HEADING BOX.
\headsep     .03\paperheight	% VERT. SPACE BETWEEN HEAD AND TEXT.
\footskip    .04\paperheight	% FROM END OF TEX TO BASE OF FOOTER. (40pt)
\marginparsep 9\p@		% HOR. SPACE BETWEEN TEXT AND MARGINAL NOTE
\marginparpush 6\p@		% MIN. VERT. SPACE BETWEEN MARGINAL NOTES
\hoffset -1in				% TO ADJUST WITH PAPER:
\oddsidemargin .14\paperwidth	% LEFT MARGIN FOR ODD PAGES (20)
\evensidemargin .14\paperwidth	% LEFT MARGIN FOR EVEN PAGES (20)
\marginparwidth .11\paperwidth	% TEXTWIDTH OF MARGINALNOTES



% Header and footer
\def\ps@PoS{%
  \def\@oddfoot{%
    \ifnum\value{page}=1
    % copyright and link on front page footer
	\PoScopyright@box\hfill%
	\tiny\posurl%
	\else%
    % page numbers on all other pages footers
    \reset@font\hfil\thepage\hfil%
    \fi}%
  \def\@oddhead{%
    \ifnum\value{page}=1
    % logo on first page header
    \smash{\makebox[0cm][l]{\logo}}\hfill%
    \else%
    % running headers on all other pages
    \smash{\vbox{\hsize=\textwidth\noindent
	    \ifshorttitle{\small\it\@shorttitle}\else{\small\it\@title}\fi\hfill
	    \printHeadAuthors\vskip.17em \hrule }}%
    \fi}%
  \let\@mkboth\@gobbletwo  %%%%
  \let\sectionmark\@gobble
  \let\subsectionmark\@gobble
}


% Define all our variables as empty
\def\@subheader{\@empty}
\def\@abstract{\@empty}
\def\@xtum{\@empty}
\def\@accepted{\@empty}
\def\@received{\@empty}
\def\@revised{\@empty}
\def\@published{\@empty}
\def\doi@url{\@empty}
\def\doi@anchor{\@empty}
\def\@dedicated{\@empty}
\def\@shorttitle{\@empty}
\def\@afterAbstractEmitNotes{\@empty}

\def\logo{\raisebox{-5mm}{\hbox{\noindent\includegraphics{PoSlogo}}}}

% Populate variables
\newcommand{\subheader}[1]{\gdef\@subheader{#1}}
\renewcommand{\abstract}[1]{\gdef\@abstract{#1}}
\newcommand{\notes}[1]{\gdef\@afterAbstractEmitNotes{#1}}

\newcommand\dedicated[1]{\gdef\@dedicated{\vskip .5\titlesk@c
                               \vbox{\small\it\raggedleft #1}}}

\newcommand{\ShortTitle}[1]{\gdef\@shorttitle{#1}\shorttitletrue}

\gdef\FullConference@box{\relax}
\newif\ifMissingFullConference\MissingFullConferencetrue
\newcommand\FullConference[1]{\gdef\FullConference@box{
			 \vbox{\small\raggedright
			   \it #1}}%
\MissingFullConferencefalse}

% wrap table of content with two lines
% also make it just after the title page
\let\oldTableofcontents\tableofcontents
\renewcommand\tableofcontents{\dotoctrue}

%comodity (just to have always the same spelling and layout)
\newcommand\acknowledgments{\section*{Acknowledgments}}
\newcommand\posurl{\url{https://pos.sissa.it/}}

%% add some footnotetext without the footnotemark
%% (change the mark and step the counter depending on optional argument)
\newcommand\note[2][?]{%
  \begin{NoHyper}
    %% with empty optional argument, add a footnote text without any footnotemark
    \if!#1!%
      \let\thefootnote\relax\footnotetext{#2}%
    \else
      %% in any other case, step the footnote counter
      \stepcounter{footnote}%
      %% if an optional argument was NOT given, add a default footnotetext
      \if?#1%
      \footnotetext{#2}%
      \else%
      %% if an optional argument WAS given, add a footnotetext using the argument as mark
      \renewcommand{\thefootnote}{#1}\footnotetext{#2}%
      \fi%
    \fi%
    \let\thefootnote\oldthefootnote%
  \end{NoHyper}
}


% Copyright
\gdef\PoScopyright@box{\parbox[b]{.7\textwidth}{\tiny $\copyright$ Copyright owned by the
author(s) under the terms of the Creative Commons\\
Attribution-NonCommercial-NoDerivatives 4.0 International
License (CC BY-NC-ND 4.0).}}


% Affiliations
\newtoks\affil@toks\newif\ifaffil\affilfalse
\newcommand{\affiliation}[2][]{%
\affiltrue
  \if!#1!%
    \affil@toks=\expandafter{\the\affil@toks{\item[]#2}}%
  \else
    \affil@toks=\expandafter{\the\affil@toks{\item[$^{#1}$]#2}}%
  \fi
}

% E-mails
% (automatically add a comma between emails)
\newtoks\email@toks\newcounter{email@counter}%
\setcounter{email@counter}{0}%
\newcommand{\emailAdd}[1]{%
\emailaddtrue%
\ifnum\theemail@counter>0\email@toks=\expandafter{\the\email@toks, \@email{#1}}%
\else\email@toks=\expandafter{\the\email@toks\@email{#1}}%
\fi\stepcounter{email@counter}}
\newcommand{\@email}[1]{\href{mailto:#1}{#1}}


\renewcommand{\@dotsep}{10000}

% Hooks after various pieces of the title page
% (these hooks also define the spacing between the pieces)
\newlength{\affiliationsSep}\setlength{\affiliationsSep}{-3pt}
\newcommand{\hookBeforeTitle}{\vskip2em   plus .4fill  minus 1em}
\newcommand{\hookAfterTitle}{\vskip1.7em plus .1fill  minus 1em}
\newcommand{\hookAfterRule}{\vskip1.7em plus .1fill  minus 1em}
\newcommand{\hookAfterAuthor}{\relax}
\newcommand{\hookAfterAffiliation}{\relax}
\newcommand{\hookAfterEmail}{\vskip16pt plus0.2fill minus10pt\filbreak}
\newcommand{\hookAfterAbstract}{\vskip1.5em plus .05fill minus 1em}
\newcommand{\hookAfterToc}{\vskip 2em \@plus 3ex \@minus 3ex}
\newcommand{\hookAfterTocRule}{\vskip 2em \@plus 3ex \@minus 3ex}

\newcommand{\PoSTOCrule}{\noindent\rule\textwidth{.1pt}}

\renewcommand\maketitle{\pagestyle{PoS}%
  \begingroup%
  \renewcommand\thefootnote{\@fnsymbol\c@footnote}%
  \begin{flushleft}%				% PAY ATTENTION TO \par'S
    \null
    %
    \hookBeforeTitle
    %
    {\LARGE\sffamily              % TITLE
      \bfseries\boldmath
      \@title\par}%
    %
    \hookAfterTitle
    %
    \hrule height 1\p@%            % RULE  1pt.
    %
    \hookAfterRule
    %
           {%
             \raggedright%
             \renewcommand\baselinestretch{1.2}%
             \bfseries%
             \sffamily%
             \large%
             \printAuthors%
             \par
           }
    %
    \hookAfterAuthor
    % Affiliations
    \ifaffil\begin{list}{}{%
      \setlength{\leftmargin}{0.28cm}%
      \setlength{\labelsep}{0pt}%
      \setlength{\labelwidth}{1em}%
      \setlength{\itemsep}{\affiliationsSep}%
      \setlength{\topsep}{-\parskip}}
    \itshape\small%
    \the\affil@toks
    \end{list}\fi
    %
    \hookAfterAffiliation
    %
    \ifemailadd %% if emailadd is true
    \noindent\hspace{0.28cm}\begin{minipage}[l]{.9\textwidth}
      \begin{flushleft}
        \textit{E-mail:} {\ttfamily\small\the\email@toks}
      \end{flushleft}
    \end{minipage}\fi
    %
    \hookAfterEmail
    %
    % abstract (narrower)
    \if!\@abstract!\else%
    \noindent\hspace{0.28cm}% same indent as affiliations and email (TODO: parametrize indent)
    \parbox{.9\textwidth}{\small\ignorespaces\@abstract\normalsize}%
    \fi%
    \@afterAbstractEmitNotes%
    %
    \@dedicated                     % DEDICATION (if present) with its space
    %
    \hookAfterAbstract
    \vfill
    \FullConference@box            % FULL CONFERENCE INFO
  \end{flushleft}%
  %
  \newpage				% END OF PAGE
  \endgroup
  \flushbottom
  \setcounter{footnote}{0}%
  \ifdotoc%
      \PoSTOCrule
      \hookAfterTocRule
      \oldTableofcontents
      \hookAfterToc
      \PoSTOCrule
      \hookAfterTocRule
  \fi%
  \ifMissingFullConference%
  \PackageWarningNoLine{pos}{No conference info. Please use the macro \protect\FullConference}%
  \fi%
}
%%%%%%%%%%%%%%%%%%%%%%%%%% ACTUAL TITLEPAGE %%%%%%%%%%%%%%%%%%%%%%%%%%%


\setcounter{secnumdepth}{3}

\newcommand\secstyle{\bfseries\raggedright}

\renewcommand\section{\@startsection{section}{1}{\z@}%
                                   {3.5ex \@plus 1.3ex \@minus .7ex}%
                                   {2.3ex \@plus.4ex \@minus .4ex}%
                                   {\normalfont\large\secstyle}}
\renewcommand\subsection{\@startsection{subsection}{2}{\z@}%
                                   {2.3ex\@plus 1ex \@minus .5ex}%
                                   {1.2ex \@plus .3ex \@minus .3ex}%
                                   {\normalfont\normalsize\secstyle}}
\renewcommand\subsubsection{\@startsection{subsubsection}{3}{\z@}%
                                   {2.3ex\@plus 1ex \@minus .5ex}%
                                   {1ex \@plus .2ex \@minus .2ex}%
                                   {\normalfont\normalsize\secstyle}}
\renewcommand\paragraph{\@startsection{paragraph}{4}{\z@}%
                                   {1.75ex \@plus1ex \@minus.2ex}%
                                   {-1em}%
                                   {\normalfont\normalsize\bfseries}}
\renewcommand\subparagraph{\@startsection{subparagraph}{5}{\parindent}%
                                   {1.75ex \@plus1ex \@minus .2ex}%
                                   {-1em}%
                                   {\normalfont\normalsize\bfseries}}

%% append a dot after the section number
%% (only for sections, not for sub-sections etc.)
%% https://texfaq.org/FAQ-seccntfmt
%% https://tex.stackexchange.com/a/24444/56076
\newcommand*{\adddot@section}{.}
\renewcommand*{\@seccntformat}[1]{%
  \csname the#1\endcsname
  \csname adddot@#1\endcsname\hspace{1ex}
}

